Verification of agent knowledge in dynamic access control policies

We develop a modeling technique based on interpreted systems in order to verify temporal-epistemic properties over access control policies. This approach enables us to detect information flow vulnerabilities in dynamic policies by verifying the knowledge of the agents gained by both reading and reasoning about system information. To overcome the practical limitations of state explosion in model-checking temporal-epistemic properties, we introduce a novel abstraction and refinement technique for temporal-epistemic safety properties in ACTLK (ACTL with knowledge modality K) and a class of interesting properties that does fall in this category.

==> Requirements/Requirements.tex <==
\section{Requirements in modelling access control systems in IS framework}
\label{sec:modelling}

Multi-agent access control systems grant or deny user access to the resources and services depending on the access rights defined in the policy. Access to the resources is divided into \emph{write access}, which when granted, allows updating some system variables (in the context of this work, Boolean variables) and \emph{read access}, that returns the value of some variables when granted. 

By definition \cite{NIST-assessment}, a \emph{safe} access control system does not leak permissions to an unauthorized principal. Information flow analysis investigates the possibility of gaining information by unauthorized agents. An intruder may gain information by directly accessing or by reasoning about the information. Modelling access control systems using interpreted systems framework enables us to reason about agents' knowledge and find information flow vulnerabilities caused by reasoning.

\subsection{Temporary read permissions}
\label{sec:dynamiclocal}

In access control systems, we deal with read and write access procedures. Write procedures, which update a set of variables, are contained in interpreted systems as actions. In interpreted systems, a principal knows a fact if it is included in his local state or he can deduce it by applying logical reasoning. In access control systems and in addition to the local information, agents may obtain permission to directly access some resources in the system. This perission may be granted by the system or other agents (delegation of authority). For instance, in a web application users always have access to their own profile, but they cannot access to the other users' profile unless the permission is granted by the owners. When a read permission to a resource is granted, the resource will become a part of agent's local state. When the permission is denied, it will be removed from agent's directly accessible information. This behaviour is similar to a system which uses dynamically changing local states to model permissions.

Interpreted systems formally contain local states which cannot change during execution of the system. In order to model temporary read permissions, we need to introduce some locally accessible information, which simulates the temporary read access. We will explain how to introduce temporary read permissions when modelling access control systems in section \ref{sec:buildis}.

\subsection{Asynchronous actions}

In interpreted systems, the agents perform actions (including $\Lambda$ as \emph{no operation}) in each clock cycle. In a \emph{synchronous systems}  agents can perform actions in parallel in each clock cycle, whereas in an \emph{asynchronous systems} only one of the agents performs a non-$\Lambda$ action per clock cycle. One of the common problems in synchronous systems is the \emph{race condition}. Race condition may result in some unwanted situations that we are not interested to face when verifying access control systems.

In our approach, we are \emph{not} interested in security breaches caused by a race condition. We consider that such issues are handled by memory locks or other application level methods. In general and in real systems, different requests are held in a queue and processed one at a time asynchronously. So, it is a realistic approach to model access control systems in asynchronous manner.

\begin{definition}[Asynchronous system]
An interpreted system is \emph{asynchronous} if all joint actions contain at most one non-$\Lambda$ agent action.
\end{definition}

